Green Security Game with Community Engagement

While game-theoretic models and algorithms have been developed to combat illegal activities, such as poaching and over-fishing, in green security domains, none of the existing work considers the crucial aspect of community engagement: community members are recruited by law enforcement as informants and can provide valuable tips, e.g., the location of ongoing illegal activities, to assist patrols. We fill this gap and (i) introduce a novel two-stage security game model for community engagement, with a bipartite graph representing the informant-attacker social network and a level-$\kappa$ response model for attackers inspired by cognitive hierarchy; (ii) provide complexity results and exact, approximate, and heuristic algorithms for selecting informants and allocating patrollers against level-$\kappa$ ($\kappa<\infty$) attackers; (iii) provide a novel algorithm to find the optimal defender strategy against level-$\infty$ attackers, which converts the problem of optimizing a parameterized fixed-point to a bi-level optimization problem, where the inner level is just a linear program, and the outer level has only a linear number of variables and a single linear constraint. We also evaluate the algorithms through extensive experiments.

==> chapters/levelkattacker.tex <==
\section{Defending Against Level-$\kappa$ Attackers}
In the previous section, we deal with the case with only type-0 attackers and provide algorithms to find the optimal set of informants to recruit. In this section, we show how those approaches can be easily extended to the case with level-$\kappa$ attackers.

Once given $\bx_{\kappa}$, $\bq^{\kappa}$ can be easily obtained. So as $\DefEU_{\kappa}$, the defender's expected utility when using $\bx_{\kappa}$ against a single attack of a level-$\kappa$ attacker. To get the solution, we simply replace $\DefEU_{0},\bq^0$ with $\DefEU_{\kappa},\bq^{\kappa}$ and apply \Select or \Heuristic.
In order to calculate $\bx_{\kappa}$ by definition, all that remains is to calculate $\MS(\bx_i,\bx, \bq_i)$ for $i<\kappa$, which could be done by a enumeration of all tip combinations. %and find the strategy for each combination following Theorem \ref{thmalloc}.
